Next generation input-output data format for HEP using Google's protocol buffers

We propose a data format for Monte Carlo (MC) events, or any structural data, including experimental data, in a compact binary form using variable-size integer encoding as implemented in the Google's Protocol Buffers package. This approach is implemented in the so-called ProMC library which produces smaller file sizes for MC records compared to the existing input-output libraries used in high-energy physics (HEP). Other important features are a separation of abstract data layouts from concrete programming implementations, self-description and random access. Data stored in ProMC files can be written, read and manipulated in a number of programming languages, such C++, Java and Python.

==> Makefile <==
###############################################################################
#
# Makefile for the photon note
#                              	
###############################################################################

NOTENAME=promc


all:#default target makes everything
	latex $(NOTENAME).tex && bibtex $(NOTENAME) && latex $(NOTENAME).tex && latex $(NOTENAME).tex && dvips -P pdf $(NOTENAME).dvi && ps2pdf $(NOTENAME).ps $(NOTENAME).pdf

dvi:
	latex $(NOTENAME).tex && bibtex $(NOTENAME) && latex $(NOTENAME).tex 

ps:
	latex $(NOTENAME).tex && bibtex $(NOTENAME) && latex $(NOTENAME).tex && latex $(NOTENAME).tex && dvips -P pdf $(NOTENAME).dvi 

pdf:
	latex $(NOTENAME).tex && bibtex $(NOTENAME) && latex $(NOTENAME).tex && latex $(NOTENAME).tex && dvips -P pdf $(NOTENAME).dvi && ps2pdf $(NOTENAME).ps $(NOTENAME).pdf

show:
	evince $(NOTENAME).pdf

.PHONY: clean
clean:
	rm -rf $(NOTENAME).aux $(NOTENAME).log $(NOTENAME).out $(NOTENAME).bbl $(NOTENAME).blg\
	$(NOTENAME).dvi $(NOTENAME).ps \
	$(NOTENAME).toc $(NOTENAME).tof thumb*.* *~ 

